A Framework for the Analysis of Computational Imaging Systems with Practical Applications

Over the last decade, a number of Computational Imaging (CI) systems have been proposed for tasks such as motion deblurring, defocus deblurring and multispectral imaging. These techniques increase the amount of light reaching the sensor via multiplexing and then undo the deleterious effects of multiplexing by appropriate reconstruction algorithms. Given the widespread appeal and the considerable enthusiasm generated by these techniques, a detailed performance analysis of the benefits conferred by this approach is important. Unfortunately, a detailed analysis of CI has proven to be a challenging problem because performance depends equally on three components: (1) the optical multiplexing, (2) the noise characteristics of the sensor, and (3) the reconstruction algorithm. A few recent papers have performed analysis taking multiplexing and noise characteristics into account. However, analysis of CI systems under state-of-the-art reconstruction algorithms, most of which exploit signal prior models, has proven to be unwieldy. In this paper, we present a comprehensive analysis framework incorporating all three components. In order to perform this analysis, we model the signal priors using a Gaussian Mixture Model (GMM). A GMM prior confers two unique characteristics. Firstly, GMM satisfies the universal approximation property which says that any prior density function can be approximated to any fidelity using a GMM with appropriate number of mixtures. Secondly, a GMM prior lends itself to analytical tractability allowing us to derive simple expressions for the `minimum mean square error' (MMSE), which we use as a metric to characterize the performance of CI systems. We use our framework to analyze several previously proposed CI techniques, giving conclusive answer to the question: `How much performance gain is due to use of a signal prior and how much is due to multiplexing?

==> extraSimuFigs.tex <==
%\begin{figure*}[tbh]
%	\centering
%		\includegraphics[width=2\columnwidth]{figures/compareEDOFsystems/compareEDOFsimuLowLightNew.pdf}
%\vspace{-.1in}
%	\caption{\emph{Simulation results for EDOF systems at low light condition (photon to read noise ratio of $J/\sigma^2=0.2$).} Using GMM prior, focal sweep \cite{Nagahara:08}, wavefront coding \cite{dowski1995extended} and coded aperture design of Levin \cite{levin2007image} produce SNR gains (w.r.t. impulse systems) of $7.5$ dB, $10.9$ dB and $3.5$ dB respectively. Also, note that for the impulse system and coded aperture of Levin, GMM and BM3D give similar reconstruction SNR, where as for the focal sweep and wavefront coding BM3D reconstructions are $~2$ dB better than the GMM reconstruction.}
%\label{fig:compareEDOFsimuLowLight}
%\vspace{-.2in}
%\end{figure*}

%\begin{figure*}[tbh]
%	\centering
%		\includegraphics[width=2\columnwidth]{figures/compareMotionDeblurSystems/compareMotDeblurSimuLowLightNew.pdf}
%\vspace{-.1in}
%	\caption{\emph{Simulation results for motion deblurring systems at low light condition (photon to read noise ratio of $J/\sigma^2=0.2$).} Using GMM prior, flutter shutter \cite{raskar2006coded} and motion invariant system \cite{levin2008motion} produce SNR gains (w.r.t. impulse systems) of $4$ dB and $7.7$ dB respectively. For the impulse system, GMM reconstruction is $3.4$ dB better than the BM3D reconstruction, where as for the flutter shutter and motion invariant system, GMM and BM3D produce similar results. }
%\label{fig:compareMotDeblurSimuLowLight}
%\vspace{-.2in}
%\end{figure*}

%\begin{figure*}[tbh]
%	\centering
%		\includegraphics[width=2\columnwidth]{figures/compareLFSystems/compareLFSimuLowLight.pdf}
%\vspace{-.1in}
%	\caption{\emph{Simulation results forlight field cameras at low light condition (photon to read noise ratio of $J/\sigma^2=0.2$).} Using GMM prior, Lytro \cite{ng2005light} and the programmable aperture camera \cite{liang2008programmable} produce SNR gains (w.r.t. impulse systems) of dB and dB respectively.}
%\label{fig:compareLFSimuLowLight}
%\vspace{-.2in}
%\end{figure*}



==> optParamSetting.tex <==
\begin{figure}[htb]
	\centering
		\includegraphics[width=3.5in]{figures/OptSetting/motionDeblurring.png}
	\label{fig:motionDeblurring}
	\caption{\emph{Optimal exposure setting for motion deblurring:} Depending on the range of object velocities we want to capture, we first fix the exposure setting of the impulse imaging in such a way that the motion blur is less than a pixel. We then analytically compute the expected SNR gain of different exposure settings (PSF kernel lengths) with respect to the  impulse imaging system (of PSF kernel length $1$)  at various light levels, see subplot (a). For light levels less than $150$ lux capturing the image with a larger exposure and then deblurring is a better option, whereas, for light levels greater than $150$ lux we should always capture impulse image and then denoise. Subplot (b) shows the optimal blur PSF length at different light levels. At light level of $1$ lux, the optimal PSF is $23$, whereas for light levels greater than or equal to $150$ lux the optimal is $1$, i.e., the impulse image setting. Subplots (c-e) show the simulated results with different PSF kernel lengths at a few lighting levels.}
\end{figure}

We use our analytic lower bound for MMSE to compute the optimal parameter setting of conventional camera for motion and defocus deblurring. The optimal parameters, exposure for motion deblurring and aperture for defocus deblurring, obviously depends on the scene light level. Hence, we compute the optimal parameters as a function of light levels.

\subsection{Optimal Exposure Setting for Motion Deblurring}
We first fix the exposure setting of the impulse imaging system based on the range of object velocities we want to capture. The exposure is set to a value that the motion blur for the desired range of velocities is less than a pixel. We then analytically compute the expected SNR gain of different exposure settings (PSF kernel lengths) with respect to the  impulse imaging system (of PSF kernel length $1$)  at various light levels, see Figure \ref{fig:motionDeblurring}(a). For light levels less than $150$ lux capturing the image with a larger exposure and then deblurring is a better option, whereas, for light levels greater than $150$ lux we should capture the impulse image and then denoise. Figure \ref{fig:motionDeblurring}(b) shows the optimal blur PSF length at different light levels. At light level of $1$ lux, the optimal PSF length is $23$, whereas for light levels greater than or equal to $150$ lux the optimal length is $1$, i.e., the impulse image setting. Figure \ref{fig:motionDeblurring} (c-e) show the simulated results with different PSF kernel lengths at a few lighting levels.

\begin{figure}[htb]
	\centering
		\includegraphics[width=3.5in]{figures/OptSetting/defocusDeblurring.png}
	\label{fig:defocusDeblurring}
	\caption{\emph{Optimal aperture setting for defocus deblurring:} Depending on the desired DOF, we fix the aperture size of the impulse imaging system so that the defocus blur is less than a pixel. We then analytically compute the SNR gain of different aperture settings (PSF kernel size) with respect to impulse imaging system of PSF kernel size $1\times1$ for various light levels, see subplot (a). For light levels less than $400$ lux capturing the image with a larger aperture and then deblurring is a better option, whereas, for light levels greater than $400$ lux we should capture impulse image and then denoise. In subplot (b) we show the optimal blur PSF size at different light levels. At light level of $1$ lux, the optimal PSF is $9\times9$, whereas for light levels greater than $400$ lux the optimal is $1\times1$, i.e., the impulse image setting. Subplots (c-d) show the simulated results with different PSF size at a few lighting levels.}
\end{figure}


\subsection{Optimal Aperture Setting For Defocus Deblurring}
\label{sec:OptAperSetting}
Depending on the desired DOF, we fix the aperture size of the impulse imaging system so that the defocus deblur is less than a pixel. We then analytically compute the SNR gain of different aperture settings (PSF kernel size) with respect to impulse imaging system of PSF kernel size $1\times1$ for various light levels, see Figure \ref{fig:defocusDeblurring}(a). From this plot, we conclude that for light levels less than $400$ lux capturing the image with a larger aperture and then deblurring is a better option, whereas, for light levels greater than $400$ lux we should capture the impulse image and then denoise. Figure \ref{fig:defocusDeblurring}(b) shows the optimal blur PSF size at different light levels. At light level of $1$ lux, the optimal PSF is $9\times9$, whereas, for light levels greater than $400$ lux the optimal is $1\times1$, i.e., the impulse image setting. Figure \ref{fig:defocusDeblurring}(c-d) show the simulated results with different PSF size at a few lighting levels.


